Racing the Market: An Industry Support Analysis for Pricing-Driven DevOps in SaaS

The SaaS paradigm has popularized the usage of pricings, allowing providers to offer customers a wide range of subscription possibilities. This creates a vast configuration space for users, enabling them to choose the features and support guarantees that best suit their needs. Regardless of the reasons why changes in these pricings are made, the frequency of changes within the elements of pricings continues to increase. Therefore, for those responsible for the development and operation of SaaS, it would be ideal to minimize the time required to transfer changes in SaaS pricing to the software and underlying infrastructure, without compromising the quality and reliability.% of the service; %i.e., this development and operation should be Pricing-Driven. This work explores the support offered by the industry for this need. By modeling over 150 pricings from 30 different SaaS over six years, we reveal that the configuration space grows exponentially with the number of add-ons and linearly with the number of plans. We also evaluate 21 different feature toggling solutions, finding that feature toggling, particularly permission toggles, is a promising technique for enabling rapid adaptation to pricing changes. Our results suggest that developing automated solutions with minimal human intervention could effectively reduce the time-to-market for SaaS updates driven by pricing changes, especially with the adoption of a standard for serializing pricings.

==> alternativeTable.tex <==
\begin{table}[ht]
     \centering
     \scalebox{0.7}{
     \begin{tabular}{|l|l|l|l|l||l|l|l|l||l|l|l|l||l|l|l|l||l|l|l|l||l|l|l|l|l|l|l||l|l|l|l||l|l|l|l|}
         \hline
         \textbf{SaaS}          & \multicolumn{4}{|c||}{\textbf{2019}} & \multicolumn{4}{c||}{\textbf{2020}}   & \multicolumn{4}{c||}{\textbf{2021}}  & \multicolumn{4}{c||}{\textbf{2022}}   & \multicolumn{4}{c||}{\textbf{2023}} & \multicolumn{4}{c|}{\textbf{2024}} \\ 
         \cline{2-25}
         &  & p & f & a &  & p & f & a &  & p & f & a &  & p & f & a &  & p & f & a &  & p & f & a \\
         \hline
         \href{https://www.box.com/pricing}{Box}        & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmar &&& & \cmark &&& \\ \hline
         \href{https://buffer.com/pricing}{Buffer}        & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://www.canva.com/pricing/}{Canva}         & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://clickup.com/pricing}{ClickUp}       & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://clockify.me/pricing}{Clockify}      & \xmark &&& & \xmark &&& & \xmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://www.crowdcast.io/pricing}{Crowdcast}   & \xmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://databox.com/pricing}{Databox}       & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://www.deskera.com/pricing}{Deskera}       & \xmark &&& & \xmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://www.dropbox.com/plans}{Dropbox}  & \xmark &&& & \xmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://evernote.com/compare-plans}{Evernote}      & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://www.figma.com/pricing/}{Figma}         & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://github.com/pricing}{GitHub}        & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://hypercontext.com/pricing}{Hypercontext}  & \xmark &&& & \xmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://www.atlassian.com/software/jira/pricing}{Jira}          & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://mailchimp.com/es/pricing/marketing/compare-plans/?currency=USD}{MailChimp}     & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://www.microsoft.com/en-us/microsoft-365/enterprise/office365-plans-and-pricing}{Microsoft 365} & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://www.notion.so/pricing}{Notion}  & \nmark &&& & \nmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://www.openphone.com/pricing}{OpenPhone}     & \xmark &&& & \xmark &&& & \xmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://www.overleaf.com/user/subscription/plans}{Overleaf}      & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://planable.io/pricing/}{Planable}      & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://www.postman.com/pricing/}{Postman}       & \xmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&&\\ \hline
         \href{https://pumble.com/pricing}{Pumble}        & \xmark &&& & \xmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&&\\ \hline
         \href{https://quip.com/about/pricing}{Quip}          & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& \\ \hline
         \href{https://www.salesforce.com/eu/sales/pricing/}{Salesforce}    & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&&\\ \hline
         \href{https://slack.com/pricing}{Slack}         & \cmark &&& & \cmark &&& & \xmark &&& & \xmark &&& & \cmark &&& & \cmark &&&\\ \hline
         \href{https://www.tableau.com/pricing/teams-orgs}{Tableau}       & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&&\\ \hline
         \href{https://trustmary.com/pricing/}{Trustmary}     & \xmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&&\\ \hline
         \href{https://userguiding.com/pricing}{UserGuiding}   & \xmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&&\\ \hline
         \href{https://www.wrike.com/comparison-table/}{Wrike}         & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&& & \cmark &&&\\ \hline
         \href{https://zapier.com/pricing}{Zapier}        & \cmark &5&19&0& \cmark &5&21&0& \xmark &&&& \cmark &4&51&0& \cmark &5&51&0 & \cmark &4&51&4\\ \hline
     \end{tabular*}   
     }
     \caption{Dataset of SaaS pricings evolution resulting from the study}
     \label{table:dataset}
 \end{table}

==> calusura-combinatoria-espacio-configuracion.tex <==
\section*{Espacio de configuración de un Pricing}
La experiencia modelando con rigor los pricings de este estudio nos permite definir el espacio de configuración de un pricing a partir de sus planes, sus add-ons y las relaciones de exclusividad y dependencia. Las primeras permiten restringir un add-on a un plan en concreto, p.e. que la característica ``pet dashboard'' está disponible sólo para 'PLATINUM', o lo que es lo mismo, que no está disponible para BASIC y GOLD (\(E("pet dashboard")= \{BASIC, GOLD\} \)). Las segundas permiten establecer una dependencia entre uno y más add-ons, p.e. \(D("pet dashboard")= \{'Smart clinic Report'\} \).  

Sea \( P = \{p_1, p_2, \ldots, p_n\} \) el conjunto de planes, \( A = \{a_1, a_2, \ldots, a_m\} \) el conjunto de add-ons, \( E = \{e_1, e_2, \ldots, e_j\} \) el conjunto de relaciones de exclusión entre planes y add-ons y \( D = \{d_1, d_2, \ldots, d_k\} \) el conjunto de dependencias entre add-ons. El espacio de configuraciones del pricing se define como el conjunto de pares (plan, add-ons) que satisfacen las restricciones. Formalmente se podría definir como:

\( Configurations(P,A,E,D) = \{(p,a) \in P \cup \emptyset \times \powerset{A} \mid isValid(p,a,E,D) \)\}

donde $is valid$ se define como\footnote{En este trabajo consideramos que el proceso de suscripción garantiza que las configuraciones son válidas, invalidas.}.

\[
\begin{aligned}
isValid(p, a, E, D) \iff & \left\{ 
    \begin{aligned}
    & p \in P \cup \{\emptyset\})                                && \text{(1)} \\
    & \land a \in \powerset{A}                                   && \text{(2) } \\
    & \land ((p \neq \emptyset) \lor (a \neq \emptyset))           && \text{(3) } \\
    & \land \forall a_i \in a, \ p \notin E(a_i)                && \text{(4) } \\
    & \land \forall a_i \in a, \ D(a_i) \subseteq a              && \text{(5)} \\
    \end{aligned} 
\right\}
\end{aligned}
\]

\begin{enumerate}
    \item Cada configuración debe contener exactamente 0 o 1 plan.
    \item Cada configuración puede tener cualquier suconjunto posible de add-ons.
   \item Cada configuración debe contener al menos un plan o un add-on. 
   \item El plan elegido no está excluido por ninguno de  \item Los add-ons elgidos satisfacen todas las relaciones de dependencia

\end{enumerate}

Para conocer el tamaño del espacio de configuraciones válidas, veremos primero el espacio sin tener en cuenta exclusiones ni dependencias. 

\subsection{Cálculo de la cardinalidad máxima}

Si no tuviesemos relaciones de exclusión ni de dependencias, el tamaño máximo del espacio de configuraciones es fácil de determinar. Equivale a  calcular la  cardinalidad de \( C \), consideramos dos casos: i) configuraciones que no contienen ningún plan, y ii) configuraciones que contienen exactamente un plan.
%&
Para el primer caso, las configuraciones son todos los subconjuntos no vacíos de \( A \), esto es \( 2^m - 1 \).
%
Para el segundo caso, por cada plan en \( P \), podemos combinarlo con cualquier subconjunto (incluido el conjunto vacío) de \( A \). Hay \( n \) planes en \( P \), y \( 2^m \) subconjuntos de \( A \). 
%
Por tanto, la cardinalidad total de \( C \) es:
%
$|C| = (2^m - 1) + n \cdot 2^m$
, que queda expresada en un único término como :

\[
|C| = 2^m - 1 + n \cdot 2^m
\]

Para el caso de Petclinic, la cardinalidad total de \( C \) es:

\[
|C| = (2^m - 1) + n \cdot 2^m = 7 + 3 \cdot 8 = 31
\]

Las combinaciones posibles son:

\begin{itemize}
    \item Configuraciones sin ningún plan:
    \begin{enumerate}
        \item \{\text{report}\}
        \item \{\text{adoption}\}
        \item \{\text{dashboard}\}
        \item \{\text{report}, \text{adoption}\}
        \item \{\text{report}, \text{dashboad}\}
        \item \{\text{adoption}, \text{dashboard}\}
        \item \{\text{report}, \text{adoption}, \text{dashboad}\}
    \end{enumerate}
    \item Configuraciones con un plan:
    \begin{enumerate}
        \item \{\text{basic}\}
        \item \{\text{basic}, \text{report}\}
        \item \{\text{basic}, \text{adoption}\}
        \item \{\text{basic}, \text{dashboard}\}
        \item \{\text{basic}, \text{report}, \text{adoption}\}
        \item \{\text{basic}, \text{report}, \text{dashboard}\}
        \item \{\text{basic}, \text{adoption}, \text{dashboard}\}
        \item \{\text{basic}, \text{report}, \text{adoption}, \text{dashboard}\}

        \item \{\text{gold}\}
        \item \{\text{gold}, \text{report}\}
        \item \{\text{gold}, \text{adoption}\}
        \item \{\text{gold}, \text{dashboard}\}
        \item \{\text{gold}, \text{report}, \text{adoption}\}
          \item \{\text{gold}, \text{report}, \text{dashboard}\}
        \item \{\text{gold}, \text{adoption}, \text{dashboard}\}
        \item \{\text{gold}, \text{report}, \text{adoption}, \text{dashboard}\}

        \item \{\text{platinum}\}
        \item \{\text{platinum}, \text{report}\}
        \item \{\text{platinum}, \text{adoption}\}
                \item \{\text{platinum}, \text{dashboard}\}
        \item \{\text{platinum}, \text{report}, \text{adoption}\}
           \item \{\text{platinum}, \text{report}, \text{dashboard}\}
        \item \{\text{platinum}, \text{adoption}, \text{dashboard}\}
        \item \{\text{platinum}, \text{report}, \text{adoption}, \text{dashboard}\}

    \end{enumerate}
\end{itemize}


\section*{Cálculo de la Cardinalidad Ajustada}

\agarcia{Con esta expresión calculamos nosotros el tamaño del espacio de configuración de los SaaS del dataset}

Siendo A(p) el conjunto de add-ons disponibles para el plan p.

\[
|C| = \sum_{p \in P} \sum_{k = 0}^{|A(p)|} \binom{|A(p)|}{k}
\]

\agarcia{Cabe destacar que esta expresión no tiene el ajuste de las restricciones del conjunto D, porque tal y como hemos modelado en Yaml4SaaS no era necesario. Sin embargo, puede ser un punto de partida}

\aruiz{habrá que dejarlo para la versión de revista el cáluclo de la cardinalidad ajustada completa. Por ahora se piodría tener el cálculo de la máxima cardinalidad, o sin tener en cuenta las exclusiones. al tener en cuenta las dependencias, se tome la aproximación de sumar configuraciones válidas (aproximación de Alejnadro) o restar de la máxima (aproximación alternativa), hay que tener en cuenta aquellas configuraciones que son válidas o invalidas poque cumplen/inclumple las dos relaciones al mismo tiempo. yo tengo una primera aproximación que para el caso de petclinic funciona. Se puede ir añadiendo al informe técnico llegado el caso}


Si no tuviésemos relaciones de exclusión ni de dependencias, el tamaño máximo del espacio de configuraciones es fácil de determinar. Equivale a calcular la cardinalidad de \( C \), considerando dos casos: i) configuraciones que no contienen ningún plan, y ii) configuraciones que contienen exactamente un plan.

Para el primer caso, las configuraciones son todos los subconjuntos no vacíos de \( A \), esto es \( 2^m - 1 \).

Para el segundo caso, por cada plan en \( P \), podemos combinarlo con cualquier subconjunto (incluido el conjunto vacío) de \( A \). Hay \( n \) planes en \( P \), y \( 2^m \) subconjuntos de \( A \).

Por tanto, la cardinalidad máxima  \( C \) es:

\[
|C| = (2^m - 1) + n \cdot 2^m
\]

Para el caso de Petclinic, donde:
\begin{itemize}
    \item \( m = 3 \) (add-ons: "Smart Clinic Report", "Pet Adoption Centre", "Pet Dashboard")
    \item \( n = 3 \) (planes: BASIC, GOLD, PLATINUM)
\end{itemize}

La cardinalidad máxima de \( C \) es:

\[
|C| = (2^3 - 1) + 3 \cdot 2^3 = 7 + 3 \cdot 8 = 31
\]

\subsubsection{Ajuste por Exclusiones}

Para determinar las configuraciones inválidas no verficar las relaciones de exclusión, procedemos como sigue:  para cada plan, identificamos los add-ons que no están disponibles para ese plan ( A \ A(p) ) y contamos cuántas configuraciones posibles incluyen estos add-ons no disponibles, haciendo estas configuraciones inválidas. Sumamos todas estas configuraciones inválidas para todos los planes, obteniendo así el total de configuraciones inválidas debido a las exclusiones. De manera más rigurosa.

\[
|C|_{\text{exclusiones}} = \sum_{p \in P} \sum_{k = 0}^{|A \setminus A(p)|} \binom{|A \setminus A(p)|}{k}
\]

En el caso de Petclinic, para los planes BASIC y GOLD, las configuraciones que incluyen "Pet Dashboard" son inválidas, y suman 8 configuraciones en total. Para el plan PLATINUM, no hay configuraciones inválidas debido a que todos los add-ons están disponibles. En concreto: :

\[
A(\text{BASIC}) = \{\text{"Smart Clinic Report"}, \text{"Pet Adoption Centre"}\}
\]
\[
A(\text{GOLD}) = \{\text{"Smart Clinic Report"}, \text{"Pet Adoption Centre"}\}
\]
\[
A(\text{PLATINUM}) = \{\text{"Smart Clinic Report"}, \text{"Pet Adoption Centre"}, \text{"Pet Dashboard"}\}
\]

\[
|C|_{\text{exclusiones}} = \sum_{k = 0}^{1} \binom{1}{k} + \sum_{k = 0}^{1} \binom{1}{k} + \sum_{k = 0}^{0} \binom{0}{k} = 2 + 2 + 1 = 5
\]
\subsubsection{Ajuste por Dependencias}

Para cada add-on \( a \) que depende de un conjunto de add-ons \( D(a) \):


Para cada add-on \( a \) que depende de un conjunto de add-ons \( D(a) \):

\[
|C|_{\text{dependencias}} = \sum_{a \in A} \left( 2^{|A \setminus \{a\}|} - 2^{|A \setminus (\{a\} \cup D(a))|} \right)
\]

Para el caso de Petclinic:
\begin{itemize}
    \item - \( D("Smart Clinic Report") = \emptyset \)
    \item - \( D("Pet Adoption Centre") = \emptyset \)
    \item - \( D("Pet Dashboard") = \{"Smart Clinic Report"\} \)
\end{itemize}

\[
|C|_{\text{dependencias}} = (2^{2} - 2^{2}) + (2^{2} - 2^{2}) + (2^{2} - 2^{1}) = 0 + 0 + 2 = 2
\]

\subsubsection{Configuraciones Inválidas por Ambas Razones}

Para evitar la doble contabilización, contamos las configuraciones que son inválidas tanto por exclusión como por dependencia:
\[
|C|_{\text{ambas}} = \sum_{p \in P} \sum_{a \in A \setminus A(p)} \left( 2^{|A \setminus \{a\}|} - 2^{|A \setminus (\{a\} \cup D(a))|} \right)
\]

Para el caso de Petclinic:

\[
|C|_{\text{ambas}} = \sum_{k = 0}^{0} \binom{0}{k} + \sum_{k = 0}^{0} \binom{0}{k} = 1 + 1 = 2
\]

\subsubsection{Cardinalidad Ajustada}

Para evitar la doble contabilización de las configuraciones inválidas tanto por exclusión como por dependencia, utilizamos la fórmula:

\[
|C|_{\text{válidas}} = |C| - (|C|_{\text{exclusiones}} + |C|_{\text{dependencias}} - |C|_{\text{ambas}})
\]

Donde:
\begin{itemize}
    \item - \(|C| = (2^m - 1) + n \cdot 2^m\)
    \item - \(|C|_{\text{exclusiones}} = 8\)
    \item - \(|C|_{\text{dependencias}} = 8\)
    \item - \(|C|_{\text{ambas}} = 4\)
\end{itemize}

Aplicando la fórmula:

\[
|C|_{\text{válidas}} = 31 - (8 + 8 - 4) = 31 - 12 = 19
\]


\begin{comment}
    
\section*{Cardinalidad del Espacio de Configuración de un Pricing}

La cardinalidad del espacio de configuración, \( \text{cardinalidadP} \), se define como el número de configuraciones válidas (pares de planes y add-ons) que satisfacen las restricciones de exclusión y dependencia.

\[
\text{cardinalidadP}(P, A, E, D) = \left| \{ (p, a) \in (P \cup \{\emptyset\}) \times \powerset{A} \mid \text{isValid}(p, a, E, D) \} \right|
\]

Para un conjunto de planes \( P \), add-ons \( A \), exclusiones \( E \) y dependencias \( D \), se calcula de la siguiente manera:

\[
\text{cardinalidadP}(P, A, E, D) = \text{configuracionesSinPlan} + \sum_{p \in P} \text{configuracionesConPlan}(p)
\]

donde:

\[
\text{configuracionesSinPlan} = \left| \{ a \in \powerset{A} \mid \forall a_i \in a, D(a_i) \subseteq a \} \right|
\]

y

\[
\text{configuracionesConPlan}(p) = \left| \{ a \in \powerset{A} \mid \forall a_i \in a, p \notin E(a_i) \land D(a_i) \subseteq a \} \right|
\]

### Ejemplo

Para ilustrar esta definición, consideremos el siguiente ejemplo:
\begin{itemize}
    \item - Planes: \( P = \{BASIC, GOLD, PLATINUM\} \)
    \item - Add-ons: \( A = \{"Smart Clinic Report", "Pet Adoption Centre", "Pet Dashboard"\} \)
    \item - Relaciones de exclusión:
    \item - \( E("Pet Dashboard") = \{BASIC, GOLD\} \)
    \item - Relaciones de dependencia:
    \item - \( D("Pet Dashboard") = \{"Smart Clinic Report"\} \)
\end{itemize}
Calculamos las configuraciones válidas y la cardinalidad total:

\[
\begin{aligned}
\text{configuracionesSinPlan} &= 5 \\
\text{configuracionesConPlan}(BASIC) &= 4 \\
\text{configuracionesConPlan}(GOLD) &= 4 \\
\text{configuracionesConPlan}(PLATINUM) &= 6 \\
\text{cardinalidadP}(P, A, E, D) &= 5 + 4 + 4 + 3 = 19
\end{aligned}
\]

Para ilustrar esta definición, consideremos el siguiente ejemplo:

\begin{itemize}
    \item Planes: \( P = \{BASIC, GOLD, PLATINUM\} \)
    \item Add-ons: \( A = \{"Smart Clinic Report", "Pet Adoption Centre", "Pet Dashboard"\} \)
    \item Relaciones de exclusión:
   \( E("Pet Dashboard") = \{BASIC, GOLD\} \)
    \item Relaciones de dependencia:  \( D("Pet Dashboard") = \{"Smart Clinic Report"\} \)
\end{itemize}

Enumeramos las configuraciones válidas para calcular la cardinalidad.

Sin plan (\( p = \emptyset \)) 5 configuraciones válidas
   \begin{itemize}
       \item \{"Smart Clinic Report"\}
       \item  \{"Pet Adoption Centre"\}
       \item  \{"Pet Dashboard"\} (no válida, falta "Smart Clinic Report")
       \item  \{"Smart Clinic Report", "Pet Adoption Centre"\}
       \item  \{"Smart Clinic Report", "Pet Dashboard"\}
       \item  \{"Pet Adoption Centre", "Pet Dashboard"\} (no válida, falta "Smart Clinic Report")
       \item \{"Smart Clinic Report", "Pet Adoption Centre", "Pet Dashboard"\}
   \end{itemize}

2. Con plan \( BASIC \). 4 configuraciones válidas
   \begin{itemize}
       \item - \( BASIC \) (sin add-ons)
       \item - \( BASIC \) + \{"Smart Clinic Report"\}
       \item - \( BASIC \) + \{"Pet Adoption Centre"\}
       \item - \( BASIC \) + \{"Pet Dashboard"\} (excluido por BASIC)
       \item - \( BASIC \) + \{"Smart Clinic Report", "Pet Adoption Centre"\}
       \item - \( BASIC \) + \{"Smart Clinic Report", "Pet Dashboard"\} (excluido por BASIC)
       \item - \( BASIC \) + \{"Pet Adoption Centre", "Pet Dashboard"\} (excluido por BASIC)
       \item - \( BASIC \) + \{"Smart Clinic Report", "Pet Adoption Centre", "Pet Dashboard"\} (excluido por BASIC)
   \end{itemize}

3. Con plan \( GOLD \). 4 configuraciones válidas
   \begin{itemize}
       \item - \( GOLD \) (sin add-ons)
       \item - \( GOLD \) + \{"Smart Clinic Report"\}
       \item - \( GOLD \) + \{"Pet Adoption Centre"\}
       \item - \( GOLD \) + \{"Pet Dashboard"\} (no válida, excluido por GOLD)
       \item - \( GOLD \) + \{"Smart Clinic Report", "Pet Adoption Centre"\}
       \item - \( GOLD \) + \{"Smart Clinic Report", "Pet Dashboard"\} (no válida, excluido por GOLD)
       \item - \( GOLD \) + \{"Pet Adoption Centre", "Pet Dashboard"\} (no válida, excluido por GOLD)
       \item - \( GOLD \) + \{"Smart Clinic Report", "Pet Adoption Centre", "Pet Dashboard"\} (no válida, excluido por GOLD)
   \end{itemize}

 4. Con plan \( PLATINUM \). 6 configuracioens válidas
\begin{itemize}
  
    \item - \( PLATINUM \) (sin add-ons)
    \item - \( PLATINUM \) + \{"Smart Clinic Report"\}
    \item - \( PLATINUM \) + \{"Pet Adoption Centre"\}
    \item - \( PLATINUM \) + \{"Pet Dashboard"\}
    \item - \( PLATINUM \) + \{"Smart Clinic Report", "Pet Adoption Centre"\}
    \item - \( PLATINUM \) + \{"Smart Clinic Report", "Pet Dashboard"\}
    \item - \( PLATINUM \) + \{"Pet Adoption Centre", "Pet Dashboard"\} (no válida, falta "Smart Clinic Report")
    \item - \( PLATINUM \) + \{"Smart Clinic Report", "Pet Adoption Centre", "Pet Dashboard"\}
\end{itemize}

Total: \( 5 + 3 + 3 + 7 = 18 \) configuraciones válidas.
\end{comment}


==> oldIntro.tex <==
\section{Introduction}

% ¿Cuál es el contexto?
The Software as a Service (SaaS) model is a distribution and licensing model in which software is delivered in the cloud on a subscription basis. Instead of purchasing and installing software locally on premises, users access the software and its features through a web browser or an Application Programming Interface (API) over the cloud \cite{cusumano2010cloud}. Thus, according to \cite{itilv4}, ``is a means of delivering value to customers by facilitating outcomes customers want to achieve, without the ownership of specific costs and risks''.

% As a service, the SaaS model ``is a means of delivering value to customers by facilitating outcomes customers want to achieve, without the ownership of specific costs and risks'' \cite{itilv4}. 

However, as the range of features offered by a service expands, the subscription price may become so expensive that some users are unwilling, or unable, to afford them. This can be explained by the Pareto's curve \cite{juran1954universals}, which states that a small selected fraction of any series of elements to be controlled, such as the pricing features, always accounts for a large fraction of effect, such as the usage time; e.g the 20\% of the features are used 80\% of the time. This leads users to prefer paying only for the features they actually use. As a response, in order to serve as many customers as possible, SaaS providers implement pricing plans (henceforth pricings); i.e structures that strategically restrict feature access depending on the plan contracted by a customer, thereby balancing affordability for users | who can choose the plan that best fits their budget and needs | and profitability for providers. This approach has become the most popular software licensing mechanism for SaaS systems due to their ability to provide a predictable revenue stream for providers while offering flexibility and scalability to users \cite{Jiang2009}. Their adoption has been pivotal in the growth and sustainability of SaaS development, representing a shift from traditional software licensing to a more dynamic and user-centric approach.

% ¿Cuál es el problema? (Pricing-driven Development and Operation)

% Despite the advantages offered by this solution, supporting the SaaS business model on pricing strategies means that market forces and strategical decisions frequently re-shape pricings, either forcing to add new features, alter usage limits, modify the structure and prices of plans, and so on. Thus, in order to sustxain competitiveness while ensuring that pricing restrictions are effectively met, the changes must be timely implemented by the developers and properly supported by both the cloud infrastructure and the architecture of the system. This process - in which business decisions influence pricing modifications, thereby initiating development efforts and changes in the architecture or deployment infrastructure - has been coined as \emph{Pricing-driven Development and Operation of SaaS}\cite{JCIS2024LONG,CAISEFORUM24}.\footnote{For the sake of brevity, we may also use Pricing-driven DevOpS to refer to this concept.}
Despite the advantages offered by this solution, supporting the SaaS business model on pricing strategies means that market forces and strategic decisions frequently re-shape pricings, either forcing the addition of new features, altering usage limits, modifying the structure and prices of plans, and so on. Thus, in order to sustain competitiveness while ensuring that pricing restrictions are effectively met, these changes must be timely implemented by developers and properly supported by both the cloud infrastructure and the service's architecture. This process ---in which business decisions influence pricing modifications, thereby initiating development efforts and changes in the architecture or deployment infrastructure--- has been coined as \emph{Pricing-driven Development and Operation of SaaS}\cite{JCIS2024LONG,CAISEFORUM24}.\footnote{For the sake of brevity, we may also use Pricing-driven DevOps to refer to this concept.}

% Motivación

The need to optimize this process has led some SaaS providers to develop their own ad-hoc solutions, which, as far as we know, do not fully automate Pricing-driven DevOps but do facilitate its implementation. However, this raises an important question: how soon will Pricing-driven Development and Operation of SaaS become unmanageable with these approaches? Currently, we lack information about critical insights that are essential to answer this question: at which rate are pricings growing?, are providers using an optimal pricing design?, and so on. As can be seen, it is evident that the SaaS domain has an imminent need of standardization in the design and modeling of pricing plans. This will facilitate the development of libraries and technologies that truly automate the operation of pricing-driven services. As a initial approach, the first meta-model to represent SaaS pricings has been proposed recently: Pricing4SaaS \cite{CAISEFORUM24}, along with a serialization in YAML: Yaml4SaaS.

% Nowadays, existing approaches to implement Pricing-driven DevOpS in the industry are ad-hoc, lacking a standardized technology to define pricing plans that SaaS can operate with autonomously. Additionally, there is a gap in our understanding of the current state of industry pricings, leaving us uncertain about: How fast do pricings grow or change? Is there a common design used by the most popular SaaS? Looking at the trend of pricing plans, how soon will managing these pricing structures with traditional approaches become unmanageable? It is therefore evident that, in the realm of SaaS, there is an imminent need for a standard model to describe pricings comprehensively ---like the OpenAPI Specification for APIs--- along with libraries and technologies that enable software to adapt to these pricings seamlessly. \agarcia{Añadiríais aquí una frase para referenciar SLA4OAI?} \japarejo{Yo diría que los autores han realizado una primera propuesta con un meta-modelo y una sintaxis concreta en yaml} Thus, examining the nature of the pricing of successful services in the industry is crucial to laying the foundation for the design and development of these future technologies.


% ¿Cuáles son las contribuciones del paper?

To validate their suitability and better understand the trends in industry pricing-driven SaaS, this paper presents a systematic analysis of 30 services over a six-years period; in doing so, the main contributions of this paper are: i) present a systematic method to analyze SaaS pricings in the industry, ii) undertake a comparative analysis of the evolution of 30 services pricings over a six-years period (2019-2024), iii) provide an open dataset of \agarcia{\#} modelled pricing structures that can be used to replicate our analysis and to be extended in further researches, and iv) validate the feasibility of both Yaml4SaaS and its underlying meta-model to capture real-world pricings, identifying their limitations and potential areas for improvement.

% As a initial approach, the first meta-model to represent SaaS pricings has been proposed recently: Pricing4SaaS \cite{CAISEFORUM24}, along with a serialization in YAML: Yaml4SaaS. Therefore, in order to validate their suitability and to better understand the trends of industry pricing-driven SaaS, the main contributions of this paper apresents: a systematic analysis of 30 services over a period of six years (2019-2024). This observational study involved modeling the available versions of these SaaS products using Yaml4SaaS \cite{CAISEFORUM24}, resulting in a comprehensive dataset of over 150 pricing structures \agarcia{Citar dataset en zenodo}. In addition, our analysis validates both Yaml4SaaS and its underlying meta-model's ability to capture real-world pricings, identifying their limitations and potential areas for improvement.

% Estructura del artículo
The remainder of this paper is structured as follows: Section \ref{section:background} provides background information on pricings in the SaaS industry, the Pricing4SaaS model, and Yaml4SaaS. Section \ref{section:experiment} presents our observational study, outlining the research questions, methodology, threats to validity, and the results of our analysis. In Section \agarcia{4}, we discuss about the feasibility of existing feature toggling configuration technologies to be applied into a pricing-driven context to automate the pricing-driven operation of a SaaS. Finally, Section \agarcia{5} concludes the paper and outlines directions for future research.

